NAS-Bench-NLP: Neural Architecture Search Benchmark for Natural Language Processing

Neural Architecture Search (NAS) is a promising and rapidly evolving research area. Training a large number of neural networks requires an exceptional amount of computational power, which makes NAS unreachable for those researchers who have limited or no access to high-performance clusters and supercomputers. A few benchmarks with precomputed neural architectures performances have been recently introduced to overcome this problem and ensure more reproducible experiments. However, these benchmarks are only for the computer vision domain and, thus, are built from the image datasets and convolution-derived architectures. In this work, we step outside the computer vision domain by leveraging the language modeling task, which is the core of natural language processing (NLP). Our main contribution is as follows: we have provided search space of recurrent neural networks on the text datasets and trained 14k architectures within it; we have conducted both intrinsic and extrinsic evaluation of the trained models using datasets for semantic relatedness and language understanding evaluation; finally, we have tested several NAS algorithms to demonstrate how the precomputed results can be utilized. We believe that our results have high potential of usage for both NAS and NLP communities.

==> assets/figure_arch_transfer.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.4\textwidth]{assets/transfer_corr.png}
\caption{Correlation of architectures' test perplexities on PTB and WikiText-2.}
\label{fig:arch_transfer}
\end{figure}

==> assets/figure_dynamic_we_eval.tex <==
\begin{figure}[!h]
\centering

\begin{subfigure}[b]{.23\linewidth} 
\includegraphics[width=\textwidth]{assets/ptb_glue.pdf}
\caption{PTB}
\end{subfigure}
\hspace{10pt}
\begin{subfigure}[b]{.23\linewidth} 
\includegraphics[width=\textwidth]{assets/wikitext2_glue.pdf}
\caption{WikiText-2}
\end{subfigure}


\caption{OX: performance of 150 random architectures on GLUE benchmark (average score across ten tasks), OY: model perplexety, red line: average SGNS performance, green line: SGNS and LSTM encoder performance}
\label{fig:dynamic_we_eval}
\end{figure}

==> assets/figure_ged.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.4\textwidth]{assets/GED.png}
\caption{Upper bound of graph edit distance histogram between 1000 random pairs of architectures.}
\label{fig:ged}
\end{figure}

==> assets/figure_loss_prediction.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.4\textwidth]{assets/prediction_loss.png}
\caption{True vs predicted final testing loss based on graph2vec features.}
\label{fig:pred_loss}
\end{figure}

==> assets/figure_merged_arch_transfer_and_ged.tex <==
\begin{figure}
\centering
\begin{minipage}{.4\linewidth}
  \centering
    \includegraphics[width=1.0\textwidth]{assets/transfer_corr.png}
    \captionof{figure}{Correlation of architectures' test perplexities on PTB and WikiText-2.}
    \label{fig:arch_transfer}
\end{minipage}%
\hspace{20pt}
\begin{minipage}{.4\linewidth}
  \centering
    \includegraphics[width=1.\textwidth]{assets/GED.png}
    \captionof{figure}{Upper bound of graph edit distance histogram between 1000 random pairs of architectures.}
    \label{fig:ged}
\end{minipage}
\end{figure}

==> assets/figure_ptb_pearson_hist.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.4\textwidth]{assets/ptb_pearson_hist.pdf}
\caption{Performance of our architectures, trained on PTB, WordSim353 and SimLex999 compared to SGNS}
\label{fig:pred_loss}
\end{figure}

==> assets/figure_wikitext2_pearson_hist.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.4\textwidth]{assets/wikitext2_pearson_hist.pdf}
\caption{Performance of our architectures, trained on WikiText2, WordSim353 and SimLex999 compared to SGNS}
\label{fig:pred_loss}
\end{figure}

==> assets/table_dynamic_we_eval.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!h]
  \caption{Extrinsic evaluation of our architectures, compared to baseline}
  \label{dynamic_we_eval}
\begin{tabular}{|l|l|l|} \hline

                            &                         & GLUE Score \\ 
\multirow{3}{*}{PTB}        & our architectures (avg) &            \\ \cline{2-3} 
                            & our architectures (max) &            \\ \cline{2-3} 
                            & SGNS                    &            \\ 
\multirow{3}{*}{WikiText-2} & our architectures (avg) &            \\ \cline{2-3} 
                            & our architectures (max) &            \\ \cline{2-3} 
                            & SGNS                    &            \\ 
\hline                            
\end{tabular}
\end{table}

==> assets/table_static_we_eval.tex <==
% \usepackage{multirow}
\begin{table}[!h]
  \caption{Intrinsic evaluation of our architectures, compared to baseline}
  \label{static_we_eval}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{}}               & \multicolumn{2}{l|}{WordSimilarity-353} & \multicolumn{2}{l|}{SimLex-999} \\ \cline{3-6} 
\multicolumn{2}{|l|}{}                                & Spearman's $\rho$     & Pearson's r     & Spearman's $\rho$ & Pearson's r \\ \hline
\multirow{3}{*}{PTB}        & our architectures (avg) &                       &                 &                   &             \\ \cline{2-6} 
                            & our architectures (max) &                       &                 &                   &             \\ \cline{2-6} 
                            & SGNS                    &                       &                 &                   &             \\ \hline
\multirow{3}{*}{WikiText-2} & our architectures (avg) &                       &                 &                   &             \\ \cline{2-6} 
                            & our architectures (max) &                       &                 &                   &             \\ \cline{2-6} 
                            & SGNS                    &                       &                 &                   &             \\ \hline
\end{tabular}
\end{table}

==> sections/8.broader_impact.tex <==
\section{Broader Impact}
\label{sec:broader_impct}

All the precomputed architectures can be re-used without the need being trained them again. Since training a neural network is a computationally intensive procedure, it consumes a substantial amount of energy and time, which is stacked into large amounts when thousands of networks are trained within NAS experiments. Moreover, only a few groups with access to supercomputers can conduct a fully-functional research of NAS methods. Thus, on a global scale, our benchmark is aimed at making NAS greener and more available to the broader community, for those researchers who don't have exceptional computational resources. In addition, a detailed analysis of the wide variety of recurrent neural networks made in our and further works can yield new insights about better architectures designs for many applications like text annotation, speech recognition, and time series forecasting. 
